Shikra: Unleashing Multimodal LLM's Referential Dialogue Magic

In human conversations, individuals can indicate relevant regions within a scene while addressing others. In turn, the other person can then respond by referring to specific regions if necessary. This natural referential ability in dialogue remains absent in current Multimodal Large Language Models (MLLMs). To fill this gap, this paper proposes an MLLM called Shikra, which can handle spatial coordinate inputs and outputs in natural language. Its architecture consists of a vision encoder, an alignment layer, and a LLM. It is designed to be straightforward and simple, without the need for extra vocabularies, position encoder, pre-/post-detection modules, or external plug-in models. All inputs and outputs are in natural language form. Referential dialogue is a superset of various vision-language (VL) tasks. Shikra can naturally handle location-related tasks like REC and PointQA, as well as conventional VL tasks such as Image Captioning and VQA. Experimental results showcase Shikra's promising performance. Furthermore, it enables numerous exciting applications, like providing mentioned objects' coordinates in chains of thoughts and comparing user-pointed regions similarities. Our code, model and dataset are accessed at https://github.com/shikras/shikra.

==> TODO.tex <==
1. OFA-Large的REC指标
2. 和Visual ChatGPT这种的区别也要讲清楚

==> figures/blank_one.tex <==
\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of a caption.  It is set in Roman so mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:onecol}
\end{figure}

==> figures/blank_two.tex <==
\begin{figure*}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of a caption.  It is set in Roman so mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:twocol}
\end{figure*}

==> sections/implementation_details.tex <==
\section{Implementation Details}
\label{sec:imple}
In this section, we introduce the implementation details of XXX-GPT.


==> tables/captioning.tex <==
\begin{table*}[h]
\centering
\small
% \renewcommand{\arraystretch}{1.23}
\renewcommand{\tabcolsep}{1.25mm}
\caption{\textbf{Comparing generalist models on Image Captioning.}
We evaluate SOTA generalist models and our Shikra-13B on COCO Cap and Flickr30k in CIDEr.
}
\begin{tabular}{l|cccccccc}
\toprule
Datasets & Shikra &  & Kosmos-1 & Flamingo-9B & Flamingo-80B & GIT & Unified-IO & VisionLLM \\
\cmidrule(lr){1-1}\cmidrule(lr){2-9}
Flickr30k   &  &   & 67.1 &  &  & 49.6 &  & \\
COCO Cap   &  & & 84.7 & 79.4 & 84.3 & & 126.8 & 114.2 \\
\bottomrule
\end{tabular}%
\label{tab:captioning}
\end{table*}

==> tables/localqa.tex <==
\begin{table}[t]
\centering
% \renewcommand{\arraystretch}{1.23}
\renewcommand{\tabcolsep}{0.7mm}
\caption{Accuracy (\%) of different models on the Local-QA \emph{test-dev} split. 
Local-QA is a pointQA dataset, where models are asked to answer questions referring to a point/box input.
The QIPBA column indicates the model input: {\bf Q}uestion, {\bf I}mage, {\bf P}oint, and/or {\bf B}ounding box. Full Img, Top-score, and Smallest are three baseline method in \citep{mani2020pointqa}.} 
\begin{tabular}{l|c|cccc}
\toprule
Model                  & \multicolumn{1}{l|}{Q/I/P/B} & Overall & Color & Action & Shape \\ \cmidrule(lr){1-6}
Full Img       & + + - -                             & 37.4   & 37.2      & 45.4       & 35.9      \\
Top-score  & + + + -                             & 44.8   & 44.4    &  62.2      & 43.4      \\
Smallest         & + + + -                             & 69.2   &  69.6     &  58.0      &  56.6      \\
\citeauthor{mani2020pointqa}    & + + + -                             & 75.0   & 75.4 & 66.4  & 56.6 \\ \cmidrule(lr){1-6}
Shikra    & + + + -                             &  63.6  & 63.8 &  60.2 & 44.7\\
Shikra    & + + - +                             &  65.4  & 65.7 & 60.2  & 50.0 \\
\bottomrule
\end{tabular}
\label{tab:localqa}
\end{table}

==> tables/vqa.tex <==
\begin{table*}[h]
\centering
\small
% \renewcommand{\arraystretch}{1.23}
\renewcommand{\tabcolsep}{1.25mm}
\caption{\textbf{Comparing generalist models on VQA.}
We evaluate SOTA generalist models and our Shikra-13B on VQAv2 \citep{antol2015vqav2} and OK-VQA \citep{marino2019ok} in Accuracy (\%).
}
\begin{tabular}{l|cccccccc}
\toprule
Datasets & Shikra  & Kosmos-1 & Flamingo-80B & Flamingo-9B & BLIP-2 & Unified-IO & VPGTrans \\
\cmidrule(lr){1-1}\cmidrule(lr){2-8}

VQAv2   & 83.27  & 51.0 & 56.3 & 51.8 & 65.2 & 77.9 & 65.2\\
OK-VQA   & 53.77  &   &  50.6 & 44.7 & 45.9 & 54.0 & 45.9  \\
\bottomrule
\end{tabular}%
\label{tab:vqa}
\end{table*}
